Efficient Out-of-Distribution Detection Using Latent Space of $\beta$-VAE for Cyber-Physical Systems

Deep Neural Networks are actively being used in the design of autonomous Cyber-Physical Systems (CPSs). The advantage of these models is their ability to handle high-dimensional state-space and learn compact surrogate representations of the operational state spaces. However, the problem is that the sampled observations used for training the model may never cover the entire state space of the physical environment, and as a result, the system will likely operate in conditions that do not belong to the training distribution. These conditions that do not belong to training distribution are referred to as Out-of-Distribution (OOD). Detecting OOD conditions at runtime is critical for the safety of CPS. In addition, it is also desirable to identify the context or the feature(s) that are the source of OOD to select an appropriate control action to mitigate the consequences that may arise because of the OOD condition. In this paper, we study this problem as a multi-labeled time series OOD detection problem over images, where the OOD is defined both sequentially across short time windows (change points) as well as across the training data distribution. A common approach to solving this problem is the use of multi-chained one-class classifiers. However, this approach is expensive for CPSs that have limited computational resources and require short inference times. Our contribution is an approach to design and train a single $\beta$-Variational Autoencoder detector with a partially disentangled latent space sensitive to variations in image features. We use the feature sensitive latent variables in the latent space to detect OOD images and identify the most likely feature(s) responsible for the OOD. We demonstrate our approach using an Autonomous Vehicle in the CARLA simulator and a real-world automotive dataset called nuImages.

==> ResponseLetter.tex <==
\setcounter{page}{1}
 \pagestyle{plain}
 \newcommand{\cAron}[1]{\todo[color=blue!10, linecolor=black!50]{\textcolor{black}{\textbf{Aron}: {#1}}}}
\newcommand{\cScott}[1]{\todo[color=green!10, linecolor=black!50]{\textcolor{black}{\textbf{Scott}: {#1}}}}
\newcommand{\Abhishek}[1]{\todo[color=orange!10, linecolor=black!50,inline]{\textcolor{black}{\textbf{Abhishek}: {#1}}}}
\setlength{\parskip}{\baselineskip}
\setlength{\parindent}{0pt}

\renewcommand{\revision}[1]{#1}


\begin{center}
\large{Response to Reviews}\\
\vspace{0.1in}
\large{\textbf{Efficient Out-of-Distribution Detection Using Latent Space of $\beta$-VAE for Cyber-Physical Systems}}\\
\vspace{0.1in}
\textbf{Manuscript ID: TCPS-2020-0079}
\end{center}

\vspace{0.5in}
Dear Editors and Reviewers,

We thank you for your time and effort for providing constructive feedback on our manuscript. We have taken care to create a major revision that we feel addresses the reviewer comments. 
Below, we provide a detailed description of how we have addressed these comments. To help you with the verification of these changes, we have addressed each comment separately, and the most important changes in the major revision of our paper are typeset in \textcolor{blue}{blue~text}. 

%We are pleased to submit a major revision of our paper for consideration in the Transaction on Cyber-Physical Systems Special Issue on Artificial Intelligence and Cyber-Physical Systems. We thank the reviewers and editors for their constructive feedback on our previous submission. Below, we provide a detailed description of how we have addressed these comments in our revision. We have addressed each comment separately, and these changes are typeset in \textcolor{blue}{blue~text}. 

We thank you again for the time that you dedicated to our paper and look forward to hearing from~you.

Sincerely,
\newline
Shreyas Ramakrishna, Zahra Rahiminasab, Gabor Karsai, Arvind Easwaran, Abhishek Dubey

% \vspace{0.5in}

\newpage
%---------------------------------------------------------------------
\section*{Response to Associate Editor}

\reviewerComment{}{%
The reviewers have concerns regarding the organization of this paper, the assumption, explanation, and complexity analysis of the proposed MIG algorithm, and comparison with state-of-the-art work. Please address all these comments and resubmit.}

\response{%
Thank you for the feedback. As suggested, we have carefully revised the paper and incorporated all the reviewers' comments. To improve the paper, we have added additional content and experiments as listed below. This has increased the length of the manuscript. We will request an increase of page limit.


The specific additions that we have made are as follows. 

\begin{enumerate}[noitemsep]
    \item \textbf{Title:}
We have  updated the title from ``Efficient Out-of-Distribution Detection and Diagnosis using Disentangled Latent Representations'' to ``Efficient Out-of-distribution Detection Using Latent Space of $\beta$-VAE for Cyber-Physical Systems''. 
\item \textbf{Introduction and Problem:} \cref{sec:intro} -  We have revised the contents of the introduction to set up the \ac{ood} detection problem and compare it to the state-of-the-art techniques. Further, we have clarified the problem specification in \cref{sec:problem}. Specific requirements for the detectors have been added as a list. Further, we have shown the effectiveness of our approach by formulating an online time series change detection problem as well. 
\item \textbf{Partial Disentanglement}: We have clarified that we are interested in achieving partial disentanglement and not full disentanglement, which is very difficult to achieve for practical datasets.  Even partial disentanglement provides good detection capabilities as shown in \cref{Table:design-space}, and aid in \ac{ood} reasoning (See \cref{fig:confidence} and \cref{fig:nuImage-confidence}).
\item \textbf{Background:} We have added a background section \cref{sec:background} which was missing in our previous version.  
\item \textbf{Design Approach:} In \cref{sec:approach-overview} we have added a design approach in \cref{fig:approach} to explain the implementation of our approach. We have clarified the  steps of the design approach in this section.  We report the complexity analysis of the MIG calculations and design space complexity of the \acl{bo} algorithm in this section.
\item \textbf{Algorithm Revision:} The \cref{algo:ld} has been modified to include the Welford's variance calculator for computing the variance of the average \ac{kl} difference across scenes. \cref{algo:MIG} has been revised based on our concept of data partitions.
\item \textbf{New figures:} We have added new figures (\ref{fig:image-features},\ref{fig:weather},\ref{fig:approach},\ref{fig:latent},\ref{fig:pipeline},\ref{Table:Train},\ref{fig:feature-variance},\ref{fig:latent-plots},\ref{fig:change-point},\ref{fig:nuImage-confidence}) to better explain our procedures.
\item \textbf{New Tables:} We have added Table \ref{Table:design-space} with new experimental results to evaluate our approach. Table \ref{Table:avgkl} has been modified to better explain the latent variable selection process.
\item \textbf{Experiments} The experiment section have been revised extensively
\begin{enumerate}[noitemsep]
\item We have clarified the difference between the test data and training data distributions using \cref{fig:feature-variance}.
\item In \cref{sec:system-setup} we have modified the data generation section to include the \acl{sdl} that we used (\cref{Table:Train}).
\item We have  introduced \cref{fig:latent-plots} and summarized results in  \cref{Table:avgkl}  to explain the effectiveness of the approach of selecting most informative latent variables. 
\item Specific experiments to show the effectiveness of our workflow (\cref{fig:approach}) compared to other approaches for training the detectors and searching the latent space were added in  \cref{Table:avgkl}.
\item  \cref{sec:nuimage} discusses the generalization of our approach to a real-world data set.
\item \cref{fig:change-point} are plots from new experiments have been added to this revision.
\end{enumerate}
\item The \textbf{discussion} and the \textbf{related research} sections have been revised as well. Specifically these new references have been added: \cite{kohli2019enabling}, \cite{dubey2011model},\cite{szegedy2013deep}, \cite{nuimage}, \cite{hartsell2021resonate}, \cite{sundar2020out}, \cite{tran2017disentangled}, \cite{peng2017reconstruction}, \cite{jakab2020partial}, \cite{mathieu2019disentangling}, \cite{hutter2019automated}, ~\cite{welford1962note}, \cite{basseville1993detection}, \cite{seto1998simplex}, ~\cite{edwards2008elements}, ~\cite{fremont2019scenic}, ~\cite{msdl}, ~\cite{dejanovic2017textx}, \cite{pan2009survey}, ~\cite{long2015learning}, \cite{heinze2021conditional}, \cite{volpi2018generalizing}, \cite{wang2019characterizing},  \cite{devries2018learning}, \cite{lakshminarayanan2016simple}, \cite{geifman2018bias}, \cite{jha2019attribution}, \cite{sundararajan2017axiomatic}, \cite{makhzani2015adversarial}, \cite{beggel2019robust}.

% We have evised the data generation section to include a \acl{sdl} that is shown in \cref{Table:Train}. Further, we have clarified the distribution change between trained and test data. We have also added \cref{fig:latent-plots}. It explains the effectiveness of our approach of selecting most informative latent variables. 

% \textbf{Experiments:} In \cref{sec:experiments} we demonstrate our approach for an \ac{av} example in CARLA simulation and a real-world automotive dataset called nuImages. In \cref{sec:system-setup} we have revised the data generation section to include a \acl{sdl} that is shown in \cref{Table:Train}. In \cref{sec:detector-design} we have added revised contents of the latent variable mapping paragraph and the results table in \cref{Table:avgkl}. We have also introduced \cref{fig:latent-plots} to explain out approach of selecting most informative latent variables. In \cref{sec:experiments} we have added additional experiments and revised its content. Specifically, we have rewritten \cref{sec:runtime-ood} to clearly explain our experiments for runtime \ac{ood} detection. \cref{fig:change-point} are plots from new experiments added to this revision of the work. \cref{sec:design-evaluation} has been a new content added to evaluate or design approach and the results are reported in \cref{Table:design-space}. \cref{sec:nuimage} discuss the newly added experiments for nuImages dataset. Further, \cref{sec:discussion} has been revised to better suite the new contents of the revised paper.
\end{enumerate}




%(3) \cref{sec:problem} - We have also revised a few paragraphs of the problem formulation section to include a new problem and included a requirements paragraph. 








%Finally, we have revised the related work in \cref{sec:RW} to include the papers suggested by the reviewers. 


}

%---------------------------------------------------------------------
%\clearpage
\section*{Response to Reviewer \#1}

\reviewerComment{}{%
It is difficult to read the paper and extract information about any new contributions that have been made by the authors. }

\response{% 
We have reorganized the paper and its contents to clarify our contributions. The novel contribution of this work is a single detector that can identify the $2$ problems discussed in the \cref{sec:intro}. Further, we provide an approach for the detector's design  (\cref{fig:approach}), and it includes dataset partitioning, latent space encoding, and latent variable mapping. We have also proposed  heuristics  for latent space encoding and latent variable mapping. 
The latent space encoding heuristic sets up disentanglement as a hyperparameter tuning problem. \acl{bo} algorithm with a disentanglement metric called  MIG is used as the objective function in the heuristic. The heuristic for latent variable mapping includes using the average \ac{kl} and the Welford's variance calculator to identify the most informative latent variables that are used for detection. We demonstrate the design approach for an \ac{av} example in the CARLA simulation and real-world automotive dataset called nuImages. Specific text from the paper that clarifies the contribution is copied below for referral.}


\paperQuote{\textbf{Contribution}: \revision{We present an  approach to generate  a partially disentangled latent space and learn an approximate mapping between the latent variables and the images features to perform anomaly detection and reasoning. The steps in our approach are data partitioning, latent space encoding, latent variable mapping, and runtime anomaly detection. To generate the partially disentangled latent space we use a \ac{bvae}, which has a gating parameter $\beta$ that can be tuned to control information flow between the features and the latent space. For a specific value of $\beta>1$, the latent space gets partially disentangled with few latent variables encoding the majority of the information about the features, while the others being less informative. For this, we provide a \acl{bo} based heuristic that sets up disentanglement as a hyperparameter tuning problem. We also provide a heuristic for latent variable mapping to select the most informative latent variables for detection and identify the latent variables sensitive to specific features, which is used for reasoning the \ac{ood} problem. Further, we evaluate how these heuristics impact the anomaly detector properties like robustness, sensitivity, and execution time. We demonstrate our approach for an \ac{av} in CARLA simulator ~\cite{dosovitskiy2017carla}, and a real-world automotive dataset called nuImages\cite{nuimage}.}}


\reviewerComment{}{The end of page 8 and the start of page 9 have been written in a smaller font for no apparent reason. This underscores the major problem with this paper, which is in its organization. }

\response{%
We have revised the paper  organization and looked for latex errors that caused the previous font size issues. The new section outline is as follows: 
}

\paperQuote{The outline of this paper is as follows. We start with describing the system model and problem formulation and detector expectations in \cref{sec:ps}. Background concepts necessary for understanding our approach are presented in \cref{sec:background}. We describe our approach in Section \ref{sec:approach}. \cref{fig:approach} presents an overview of this approach. We present  experiments and evaluation in \cref{sec:evaluation}. We conclude with discussions and a review of related work.}


\reviewerComment{}{A lot of pre-existing frameworks and techniques have been introduced and explained in the paper, but the core contribution, which is the "MIG heuristic," has not been explained in detail. There should be a clear section that discusses this "MIG heuristic" idea and relevant experimental results that show why this specific approach is better.}

\response{%
We have moved all the pre-existing concepts to the background section \cref{sec:background}. Further, we have clarified the two herusitics we use. One  is for latent space encoding (See \cref{sec:encoding}) and the other is for latent variable mapping (See \cref{sec:approach_design_2}). The first one formulates disentanglement as a hyperparameter search problem. It uses the Bayesian Optimization problem with the MIG metric for selecting the optimal \ac{bvae} hyperparameter combination (n,$\beta$) that results in a partially disentangled latent space. The second one uses the average \ac{kl} metric with Welford's variance calculator to perform latent variable mapping and identify the latent variables for $\mathcal{L}_d$ and $\mathcal{L}_f$. Each of these heuristics is explained as a step in our new workflow (See \cref{fig:approach}). Further, we have evaluated how each of these heuristics contributes towards the detector properties of robustness, sensitivity, and detection time. These evaluations are reported in \cref{Table:design-space}, and we show that using these heuristics will result in the optimal detector properties.  We include this text here for easy reference.
}

\paperQuote{Table 3. \textbf{Design Approach Evaluation}: Evaluations of how the heuristics of our design approach influence the detector properties discussed in \cref{sec:problem}. We evaluated Robustness on Nominal (Nom), High Precipitation and High Brightness (HPB), and New Road (NR) scenes. Minimum sensitivity was evaluated the on High Precipitation (HP) and High Brightness (HB) scenes (see \cref{fig:feature-variance}). Resource efficiency was measured across all scenes. The numbers in the optimization algorithm column indicate the selected hyperparameters (number of latent variables and the $\beta$). Text in green highlights the best detector properties achieved in our experiments. Text in red highlights a high detection time.}
% \paperQuote{\revision{\textbf{Implementation}: We provide an approach (See \cref{fig:approach}) to design \ac{bvae} based latent space detectors. It has design-time steps of data partitioning, latent space encoding, latent variable mapping (discussed in this section), and runtime anomaly detection (discussed in \cref{sec:anomaly-detection}). These steps work as follows: \underline{First}, we divide the multi-labeled datasets into partitions based on the variance in the feature values. A partition consists of images with one feature having higher variance in its values, irrespective of changes in the others. \underline{Second}, we generate a latent space encoding using a \ac{bvae}, which provides a gating parameter $\beta$ to control the feature information in the latent space. The value of $\beta$ and the number of latent variables ($n$) influence the level of latent space interpretability. To find the optimal hyperparameter combination we propose a heuristic that uses the \ac{bo} ~\cite{snoek2012practical} algorithm along with a disentanglement metric called \ac{mig} \cite{chen2018isolating}. \underline{Third}, we discuss a heuristic to perform latent variable mapping to identify the set of latent variables that encodes most information of the image features. These latent variables $\mathcal{L}_d$ are used as the detector. Further, we perform a \ac{kl} based sensitivity analysis to identify the latent variable(s) $\mathcal{L}_f$ in the set $\mathcal{L}_d$, that is sensitive to specific features. The latent variable(s) in $\mathcal{L}_f$ is called reasoners and is used to identify the \ac{ood} causing features. We use the detector and the reasoners to attribute if an out-of-set feature is responsible for the \ac{ood}. The rest of this section discusses these steps.}
% }


\reviewerComment{}{Please also look at a recent paper: Attribution-Based Confidence Metric For Deep Neural Networks, and contrast it with your current work.}

\response{Thank you for suggesting the paper. We have reviewed the paper and found it interesting in the context of handling susceptibility and brittleness of \acp{dnn}. The ABC metric does not require the training dataset or labels at runtime, which is an advantage as compared to our approach that compares the test images to a calibration dataset. However, it will take future investigations to identify how the approach can be extended to specific latent variable sets which are required for the multi label reasoning problem. Further, it is not clear if feature correlations will impact the attribution of features as pointed to in \cite{sundararajan2017axiomatic}. In addition, we would like to point that our approach is two folds : first the partial disentanglement and then the ICP. The ICP can be replaced by a different metric and we are investigating this as part of future work. }
%We have added the text for this paper in our related research.}
%We have closely gone through this paper and found it interesting in the context of handling susceptibility and brittleness of \acp{dnn}. The ABC metric does not require the training dataset or labels at runtime, which is an advantage as compared to our approach that compares the test images to a calibration dataset. This aspect of the ABC metric is beneficial for runtime \ac{cps} applications. However, based on our reading we are not clear on how feature correlations impact the attribution of features \cite{sundararajan2017axiomatic}, and how the multi-label reasoning problem can be solved using the ABC metric. 
%To include other related approaches that handle the susceptibility of \acp{dnn} we have expanded our related work \cref{sec:RW}.
 

\paperQuote{Recently, \citeauthor {jha2019attribution} \cite{jha2019attribution} have proposed attribution-based confidence (ABC) metric that does not require access to training data or does not need training model ensembles. It is computed by sampling in the neighborhood of high-dimensional data and then computing a score for its conformance. The metric looks robust and does not need the training data at runtime, an advantage compared to our approach. But the impact of input feature correlations and interactions on the attribution over features as shown by \citeauthor{sundararajan2017axiomatic}  \cite{sundararajan2017axiomatic} has to be investigated.   }

%\newpage
%---------------------------------------------------------------------
%\clearpage
\section*{Response to Reviewer \#2}

\reviewerComment{}{\label{c9}%
In line 29 on page 14, please provide a citation for the claim made about Exchangeability for the p-values to be independent and uniformly distributed in [0,1].}

\response{%
We thank the reviewer for the feedback. Per the reviewer's suggestions, we have added a citation to the claim about Exchangeability for the p-values to be independent and uniformly distributed in [0,1]. The change can be referred to in \cref{sec:icp}}

\paperQuote{If they are, then we can expect the p-values to be independent and uniformly distributed in [0, 1] (Theorem 8.2, ~\cite{vovk2005algorithmic}), which can be tested using the martingale.}

\reviewerComment{}{Could you explain Table 4 in more detail? It looks ambiguous when you say that
L25 has highest KL-divergence variation in C1, C2 and C3 as looking at the table, L25 has the lowest values for C1 and C2.}

\response{We have updated our latent variable mapping heuristic to use Welford's online calculator for computing the variances. So, in the updated version, the variance calculator returns the top $5$ latent variables with the highest \ac{kl} variance for each partition. Then, the latent variable with the maximum variance in each partition is chosen as the reasoner for that partition. \cref{Table:avgkl} results are now based on the revision in our heuristic. } 

% and used Welford's online calculator to compute the variance. \cref{fig:latent} shows our approach of selecting the latent variables. Based on the discussed steps in \cref{fig:latent}, we have identified the latent variables $L25$ and $L2$ for the brightness and precipitation partitions. We have also restructured the \cref{Table:avgkl} based on our update.  Further, we have introduced \cref{fig:latent-plots} to illustrate how the distributions of the selected latent variables look for the train and test data.  We include this text here for easy reference.
% }

\paperQuote{\cref{Table:avgkl} Explanation: Finally, for each partition we identified a partition latent variable set $\mathcal{L}_P$ using the welford's algorithm as discussed in \cref{sec:approach_design_2}. We chose the top $m$ = 4 latent variables using the welford's algorithm. From this we found  $\mathcal{L}_{P1}$ = $\{L_2,L_{25},L_{20},L_0,L_{29}\}$ for $P1$ and $\mathcal{L}_{P2}$ = $\{L_{25},L_{0},L_{20},L_{2},L_{29}\}$ for $P2$. The specific \ac{kl} variance of these latent variables are reported in \cref{Table:avgkl}. Then, the union of these two sets $\mathcal{L}_d$ = $\{L_{0},L_{2},L_{20},L_{25},L_{29}\}$ were used as total detector. \cref{fig:latent-plots} shows the scatter plots of the latent distributions of the selected latent variables and 5 randomly selected latent variables ($L_1,L_3,L_5,L_{15},L_{28}$) for the train images (yellow points) and the test images (green points), which are \ac{ood} with high brightness. The latent distributions of the selected latent variables highlighted in the red box form evident clusters between the train images and the test images, and these clusters have a good intra-cluster separation. But, for the other latent variables, the distributions are scattered and do not form clean clusters, and these clusters are not well separated. }

\paperQuote{We chose the latent variable with the maximum variance in the partition latent variable sets as the reasoner for each partition. We chose $L_2$ as the reasoner for the precipitation partition $P1$ and $L_{25}$ is used as the reasoner for the brightness $P2$.}


%\newpage
%---------------------------------------------------------------------
%\clearpage
\section*{Response to Reviewer \#3}

\reviewerComment{}{This study assumes that achieving a disentangled representation may lead to better OOD detection. However, this assumption is not well-motivated or justified by experiments. It may not be possible to achieve disentangled latent representation for highly non-linear neural networks [1]. Whats are the authors' thoughts on this issue. 
[1]: Locatello, Francesco, et al. "Challenging common assumptions in the unsupervised learning of disentangled representations." international conference on machine learning. PMLR, 2019. }

\response{%
Yes, we agree that the previous submission did not clearly explain the concept of disentanglement and motivate its need in our work. In this version, We have clarified that we are interested in achieving partial disentanglement and not full disentanglement, which is very difficult to achieve for practical datasets. Even partial disentanglement provides good detection capabilities as shown in \cref{Table:design-space}, and aid in \ac{ood} reasoning (See \cref{fig:confidence} and \cref{fig:nuImage-confidence}).

We also agree that achieving disentanglement is a challenging problem to solve. As discussed in ~\cite{locatello2018challenging}, performing unsupervised disentanglement is dependent on the independence of the latent features, and inductive biases of the model and data. Based on these points, we have designed a heuristic that learns disentanglement as a function of the model's hyperparameters and dataset. This approach should allow us to choose the optimal hyperparameters (n,$\beta$) in the presence of these inductive biases. Further, as real-world datasets may not have independent features, disentangling the latent distributions is not possible. However, as discussed earlier, our approach does not require the latent space to be fully disentangled; we are interested in generating the clusters of most informative and uninformative latent variables.}

\paperQuote{\textbf{This paper}: Our approach in this work is to investigate the use of disentanglement in the latent space. This idea builds upon recent progress  in structuring and disentangling the latent space ~\cite{bengio2013representation,higgins2016beta}. Effectively, the  latent space generated by the encoder of a \acl{vae} is a Gaussian mixture model of several overlapping latent variables (See \cref{fig:disentnagle}-a), each of which encodes information about the features. However, as can be seen in \cref{fig:disentnagle}-a if the variables overlap then it is hard to use them separately for anomaly detection. Disentanglement is a state of the latent space where each latent variable is sensitive to changes in only one generative feature while being invariant to changes in the others ~\cite{bengio2013representation} i.e. the large single cluster of \cref{fig:disentnagle}-a  is broken in to several smaller clusters of single latent variables if the features are independent (fully disentangled). Such, disentangled latent variables have been successfully used in several tasks like face recognition ~\cite{tran2017disentangled,peng2017reconstruction}, video predictions ~\cite{hsieh2018learning}, anomaly detection ~\cite{wang2020oiad}, etc. However, disentangling all the latent variables is challenging for real-world datasets, and is shown to be highly dependent on inductive biases of the model and data ~\cite{locatello2018challenging}, especially if the features are correlated.}

\paperQuote{However, even partial disentanglement can lead to substantial gains as shown by \citeauthor{jakab2020partial} \cite{jakab2020partial} and \citeauthor{mathieu2019disentangling} \cite{mathieu2019disentangling}. Partial disentanglement is a heuristic that group the most informative latent variables into one cluster and the remaining latent variables that are less informative into another as shown in \cref{fig:disentnagle}-c. This enables better separation in the latent space for the train and test data as shown in \cref{fig:latent-plots} of our evaluation section.
 }

\reviewerComment{}{It is not clear how to interpret Fig. 2. Whats does the color scale represent. How are the mean and variances are computed.}

\response{%
We have revised our description of the figure and provided a explanation of theses suggested missing points. We include the figure description here for easy reference.}

\paperQuote{\textbf{Visualizing Latent Space Disentanglement}: A scatter plot illustration of all the latent distributions ($\mu$, log($\sigma^2$)) generated by the encoders of \ac{bvae} with different $\beta$ values. Each color represents a latent distribution in the latent space, and $n$=30 distributions are shown in the plot. $\beta$ controls the information flow to make the latent space interpretable. For $\beta$=1, the distributions are entangled. However, for $\beta>1$, the latent distribution start to disentangle and a few latent distributions (marked inside the red circle) encoding independent latent features stay close to $\mu$=0 and log($\sigma^2$)=0, while the other distributions lie farther.Plot axis: x-axis represents the mean of the latent distributions in the range [-5,5], and the y-axis represents the log of variance in the range [-5,5].}

\reviewerComment{}{In section 1, the "generative factors" are not well defined or formulated.}

\response{%
We have revised our definitions and replaced the term "generative factor" with "feature". Since, feature is a common term, it is easier to comprehend for the readers. We have also added   \cref{fig:image-features} to illustrate the concept of features and the values they can take.}

\paperQuote{The input images can be classified as scenes, where each scene is a short time series of similar images contextualized by certain environmental features such as weather, brightness, road conditions, traffic density, among others, as shown in \cref{fig:image-features}. These features are referred to as semantic labels \cite{nuimage} or generative factors ~\cite{higgins2016beta}, and in this paper, we refer to them as features. These features can take values continuous or discrete values for generating a set of scenes (See \cref{fig:image-features})}


\reviewerComment{}{The introduction section does not explain the problem and the approach with sufficient detail.}

\response{%
We have revised the content of the introduction to better explain the \ac{ood} detection problem. We have also added a paragraph that specifically talks about our approach to address the problem. We have also revised the problem statement to formalize the problems introduced in the introduction. We add the text here for easy reference.} 

% We have revised the introduction to better explain the \ac{ood} detection problem. The text highlighted in \cref{sec:intro} can be refereed to the revisions made to set up the context and problem.}

\paperQuote{\textbf{Problem Definition:} The problem, in this case, is to identify (a) if the current operation context is \ac{ood} with the training context, and (b) which feature(s) are likely responsible for the \ac{ood}. For example, consider that if a \ac{dnn} was not trained in heavy rain, then we want to identify during operation that the \ac{ood} is due to precipitation. Besides identifying if the input is \ac{ood} with respect to the training set, it is also important to identify if the current operational input is \ac{ood} to the previous input sequence in time series. An abrupt change in the current input will increase the system's risk as illustrated in our previous work \cite{hartsell2021resonate}. So it is critical to identify these change points during operation.  Formally, we summarize the problems as follows:
\underline{\emph{Problem 1a}} - identify if the current image is \ac{ood} with respect to the training set. \underline{\emph{Problem 1b}} - identify the feature(s) most likely responsible for the \ac{ood}, and \underline{\emph{Problem 2}} - Identify if the current image is \ac{ood} to the previous sequence of images in a time series window.}

% \paperQuote{\textbf{This paper}: Our approach in this work is to investigate use of disentanglement in the latent space. This idea builds upon recent progress in structuring and disentangling the latent space ~\cite{bengio2013representation,higgins2016beta}.
% Effectively, the latent space generated by the encoder of a \acl{vae} is a Gaussian mixture model of several overlapping latent variables (See \cref{fig:disentnagle}-a), each of which encodes information about the features. However, as can be seen in \cref{fig:disentnagle}-a if the variables overlap then it is hard to use them separately for anomaly detection. Disentanglement is a state of the latent space where each latent variable is sensitive to changes in only one feature while being invariant to changes in the others ~\cite{bengio2013representation} i.e. the large single cluster of \cref{fig:disentnagle}-a is broken into several smaller clusters of single latent variables if the features are independent (fully disentangled). Such, disentangled latent variables have been successfully used in several tasks like face recognition ~\cite{tran2017disentangled,peng2017reconstruction}, video predictions ~\cite{hsieh2018learning}, anomaly detection ~\cite{wang2020oiad}, etc. However, disentangling all the latent variables is challenging for real-world datasets, and is shown to be highly dependent on inductive biases of the model and data ~\cite{locatello2018challenging}, especially if the features are correlated. }

% \paperQuote{However, even partial disentanglement can lead to substantial gains as shown by \citeauthor{jakab2020partial} \cite{jakab2020partial} and \citeauthor{mathieu2019disentangling} \cite{mathieu2019disentangling}. Partial disentanglement is a heuristic that groups the most informative latent variables into one cluster and the remaining latent variables that are less informative into another as shown in \cref{fig:disentnagle}-c. This enables better separation in the latent space for the train and test data as shown in \cref{fig:latent-plots} of our evaluation section. However, the procedures for training the disentangled space for real world CPS scenes is hard. As a result, it is one of the aspects we focus on in this paper for achieving interpretable OOD results (reasoning about OOD).}


\reviewerComment{}{Algorithm 1 seems to be very expensive as it has to train separate $\beta$-VAEs for each (n, $\beta$) combinations. How many such VAEs are trained.}

\response{%
Yes, algorithm 1 is expensive as it has to train a \ac{bvae} every iteration. The number of the \acp{bvae} trained will depend on the number of search iterations that we want to perform. We have also added the design space complexity (\cref{sec:encoding}) of our \ac{bo} algorithm and compared it against the other approaches of grid search and random search. We have also performed experiments on the \ac{bo}, grid, and random hyperparameter search algorithms in \cref{Table:comptable}. The result shows that our heuristic with \ac{bo} algorithm finds the n,$\beta$ hyperparameters that yield the maximum MIG score. It also took the shortest time (837.05) to reach the maximum MIG score as compared to 1199.51 minutes of random search and 10924.55 minutes of the grid search. For these experiments, the random and \ac{bo} algorithms were configured to run 50 iterations, whereas the grid search had to run through the entire hyperparameter search space which had 360 combinations. Our results indicate the \ac{bo} approach to yield the best hyperparameter in the shortest time. Relevant paper texts have been provided below for reference.} 


\paperQuote{\revision{\textbf{Design Space Complexity}: Searching for optimal hyperparameters is a combinatorial problem that requires optimizing an objective function over a combination of hyperparameters. In our context, the \ac{bvae} hyperparameters to be selected are n and $\beta$, and the objective function to optimize is the MIG score whose complexity we have reported in the previous section.
The range of the hyperparameters are n $\in$ $\{n_1,n_2,....,n_l\}$ and $\beta$ $\in$ $\{\beta_1,\beta_2,....,\beta_m\}$. The hyperparameter search space then becomes the Cartesian product of the two sets. In the case of the grid search, each point of this search space is explored, which requires training the \ac{bvae} network and computing the MIG metric. Grid search suffers from the curse of dimensionality since the number of evaluations exponentially grows with the size of the search space \cite{hutter2019automated}. In comparison, random search and \ac{bo} algorithm does not search the entire space but searches for a selected number of iteration $N$. While random search selects each point in the search space randomly, the \ac{bo} algorithm performs a guided search using a Gaussian process model and an acquisition function.}}

% combination of the two search spaces that is l $\times$ m.

\paperQuote{In \ac{bo} algorithm, the first $k$ iterations stabilize the Gaussian Process model using randomly selected points in the space to train a \ac{bvae} network and compute the MIG score. After these iterations, the Gaussian process model is fitted to all the previously sampled points. Then, the acquisition function based on expected improvement uses the posterior distribution of the Gaussian process model to find a new point that may optimize the MIG score. The new point is used to train a \ac{bvae} network and compute the MIG score. So, this process is repeated for $N$ iterations, and in  every iteration a \ac{bvae} network is trained and MIG score is computed as shown in \cref{algo:BO}. This intelligent search mechanism based on prior information makes the search technique efficient as it takes a smaller number of points to explore in the search space as compared to both grid search and random search \cite{snoek2012practical,hutter2019automated}. \ac{bo} algorithm has a polynomial time complexity based on the search space of the hyper-parameters \cite{hutter2019automated}. We have reported the experimental results for these three algorithms in \cref{Table:comptable}. As seen in the Table, the \ac{bo} algorithm takes the least time and iterations to select the hyperparameters that achieve an optimal MIG score.}



\reviewerComment{}{Authors are suggested to report complexity analysis for the algorithm 2 and 3.}

\response{%
We have performed complexity analysis of the MIG algorithm in \cref{sec:mig} and the design space complexity for \acl{bo} heuristic is discussed in \cref{sec:encoding}. The text for design complexity of \ac{bo} heuristic is included in the previous comment and we include the text for MIG complexity here for easy reference.}

\paperQuote{\textbf{Complexity Analysis}: The complexity of the MIG algorithm in worst case is $O(K*|\mathcal{P}|*nq * |\mathcal{F}|*|\mathcal{T}|*n^2*ns)$. Where K is the number of iterations |$\mathcal{P}$| is the number of partitions, $n$ is the number of latent variables, |$\mathcal{F}$| is the number of features considered for the calculations, nq is the number of unique values that each feature has in the partition (e.g. for a partition with brightness=10\%, and brightness=20\%, $nq$=2), ns is the number of samples generated from each latent variable, and $|\mathcal{T}|$ is the size of training data. The specific values of these parameters for the CARLA simulation example is $K=5$, $|p|=2$, $n=30$,  $\mathcal{F}=2$, $ns=500$, and $nq$=3.}


\reviewerComment{}{Minor: On page 8, the font of the text suddenly changed from line 44.}

\response{%
We have revised the paper  organization and looked for latex errors that caused the previous font size issues. }
    

==> acmart-preload-hook.tex <==
\PassOptionsToPackage{dvipsnames}{xcolor}

==> results/data1.tex <==
\footnotesize{}
% \begin{table}[t]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Feature}                         & \textbf{\begin{tabular}[c]{@{}c@{}}Training\\ Range\end{tabular}} & \textbf{Nom}        & \textbf{HP}               & \textbf{HB}               & \textbf{HPB}              & \textbf{NR}              \\ \hline
\textbf{Sun Angle}                       & 90                                                                & 90                  & 90                        & 90                        & 90                        & 90                       \\ \hline
\textbf{Cloudiness}                      & {[}0,50{]}                                                        & 25                  & 50                        & 50                        & 25                        & 50                       \\ \hline
                                         &                                                                   &                     & {\color[HTML]{009901} \textbf{40}} & {\color[HTML]{009901} \textbf{0}}  & {\color[HTML]{009901} \textbf{50}} & {\color[HTML]{009901} \textbf{0}} \\ \cline{4-7} 
\multirow{-2}{*}{\textbf{Precipitation}} & \multirow{-2}{*}{{[}0,50{]}}                                      & \multirow{-2}{*}{0} & 60                        & 0                         & 75                        & 0                        \\ \hline
                                         &                                                                   &                     & {\color[HTML]{009901} \textbf{0}}  & {\color[HTML]{009901} \textbf{25}} & {\color[HTML]{009901} \textbf{40}} & {\color[HTML]{009901} \textbf{0}} \\ \cline{4-7} 
\multirow{-2}{*}{\textbf{Brightness}}    & \multirow{-2}{*}{{[}0,50{]}}                                      & \multirow{-2}{*}{0} & 0                         & 60                        & 60                        & 0                        \\ \hline
\textbf{Road}                            & 1,2,3                                                             & 3                   & 2                         & 2                         & 2                         & 7                        \\ \hline
\end{tabular}
\normalsize{}
% \caption{\textbf{CARLA Feature space}: CARLA scenes for $\mathcal{T}$ was generated by randomly sampling the features in their training ranges. For scenes S2-S5, the features values are changed from a value in the training range to a value outside the range at t=20s. The initial values of precipitation and the brightness are highlighted in gray.}
% \label{Table:Train}
% \vspace{-0.2in}
% % \end{table}

